Cross-lingual Inflection as a Data Augmentation Method for Parsing

We propose a morphology-based method for low-resource (LR) dependency parsing. We train a morphological inflector for target LR languages, and apply it to related rich-resource (RR) treebanks to create cross-lingual (x-inflected) treebanks that resemble the target LR language. We use such inflected treebanks to train parsers in zero- (training on x-inflected treebanks) and few-shot (training on x-inflected and target language treebanks) setups. The results show that the method sometimes improves the baselines, but not consistently.

==> corr.tex <==
\usepackage{booktables}

\\begin{tabular}{lrrrrrrrrrrrr}\n\\toprule\n{} &  SuPar UAS &  SuPar LAS &    SL UAS &    SL LAS &  UM forms &  UM lemmas &  UD tr. sentences &  Feats sim. &  Lemma sim. &  WALS distance &  Avg. train &  Avg. test \\\\\n\\midrule\nSuPar UAS        &   1.000000 &   0.962886 &  0.893761 &  0.902769 & -0.153287 &  -0.315415 &          0.046677 &    0.627178 &    0.394790 &      -0.397854 &    0.177171 &   0.265583 \\\\\nSuPar LAS        &   0.962886 &   1.000000 &  0.868607 &  0.949895 & -0.129729 &  -0.252200 &          0.137852 &    0.549278 &    0.365887 &      -0.299454 &    0.159676 &   0.330838 \\\\\nSL UAS           &   0.893761 &   0.868607 &  1.000000 &  0.934281 & -0.121983 &  -0.268481 &          0.202046 &    0.570379 &    0.299072 &      -0.254910 &    0.209280 &   0.338836 \\\\\nSL LAS           &   0.902769 &   0.949895 &  0.934281 &  1.000000 & -0.132415 &  -0.242436 &          0.262361 &    0.551970 &    0.348532 &      -0.205241 &    0.223053 &   0.363078 \\\\\nUM forms         &  -0.153287 &  -0.129729 & -0.121983 & -0.132415 &  1.000000 &   0.955096 &          0.352456 &   -0.236076 &   -0.151381 &      -0.011759 &   -0.099135 &  -0.350418 \\\\\nUM lemmas        &  -0.315415 &  -0.252200 & -0.268481 & -0.242436 &  0.955096 &   1.000000 &          0.375405 &   -0.352176 &   -0.131547 &       0.038242 &   -0.017504 &  -0.377056 \\\\\nUD tr. sentences &   0.046677 &   0.137852 &  0.202046 &  0.262361 &  0.352456 &   0.375405 &          1.000000 &   -0.151791 &   -0.249818 &       0.070054 &   -0.080685 &   0.017394 \\\\\nFeats sim.       &   0.627178 &   0.549278 &  0.570379 &  0.551970 & -0.236076 &  -0.352176 &         -0.151791 &    1.000000 &    0.751487 &      -0.253516 &    0.511454 &   0.151522 \\\\\nLemma sim.       &   0.394790 &   0.365887 &  0.299072 &  0.348532 & -0.151381 &  -0.131547 &         -0.249818 &    0.751487 &    1.000000 &      -0.495717 &    0.691039 &  -0.263930 \\\\\nWALS distance    &  -0.397854 &  -0.299454 & -0.254910 & -0.205241 & -0.011759 &   0.038242 &          0.070054 &   -0.253516 &   -0.495717 &       1.000000 &   -0.146264 &   0.456078 \\\\\nAvg. train       &   0.177171 &   0.159676 &  0.209280 &  0.223053 & -0.099135 &  -0.017504 &         -0.080685 &    0.511454 &    0.691039 &      -0.146264 &    1.000000 &  -0.210828 \\\\\nAvg. test        &   0.265583 &   0.330838 &  0.338836 &  0.363078 & -0.350418 &  -0.377056 &          0.017394 &    0.151522 &   -0.263930 &       0.456078 &   -0.210828 &   1.000000 \\\\\n\\bottomrule\n\\end{tabular}\n
